Parameterized Max Min Feedback Vertex Set

Given a graph $G$ and an integer $k$, Max Min FVS asks whether there exists a minimal set of vertices of size at least $k$ whose deletion destroys all cycles. We present several results that improve upon the state of the art of the parameterized complexity of this problem with respect to both structural and natural parameters. Using standard DP techniques, we first present an algorithm of time $\textrm{tw}^{O(\textrm{tw})}n^{O(1)}$, significantly generalizing a recent algorithm of Gaikwad et al. of time $\textrm{vc}^{O(\textrm{vc})}n^{O(1)}$, where $\textrm{tw}, \textrm{vc}$ denote the input graph's treewidth and vertex cover respectively. Subsequently, we show that both of these algorithms are essentially optimal, since a $\textrm{vc}^{o(\textrm{vc})}n^{O(1)}$ algorithm would refute the ETH. With respect to the natural parameter $k$, the aforementioned recent work by Gaikwad et al. claimed an FPT branching algorithm with complexity $10^k n^{O(1)}$. We point out that this algorithm is incorrect and present a branching algorithm of complexity $9.34^k n^{O(1)}$.

==> Sections/backup_claim.tex <==
    \begin{claim}
        $G[B_t^{\downarrow} \setminus \bar{S}]$ is acyclic.
    \end{claim}

    \begin{claimproof}
        We start with the following definition of which we will make use in our proof.

        \todo[inline]{\manolis{Add sth about the last-to-exit and first-to-enter from every component,
        as well as high livel intuition and discussion.}}

        \begin{definition}[Swap]\label{definition:swap}
            Let $w_1 - v_1 - \ldots - v_m - w_2$ be $m+2$ consecutive vertices of a cycle in
            $G[B_t^{\downarrow} \setminus \bar{S}]$, \manolis{with $m \ge 1$}.
            We will say that a \emph{swap} is happening between $w_1$ and $w_2$ if:
            \begin{itemize}
                \item $\{v_1, \ldots, v_m\} \subseteq B_t$ and 
                \item no connected component of either $G[B_{t_1}^{\downarrow} \setminus \bar{S_1}]$ or
                $G[B_{t_2}^{\downarrow} \setminus \bar{S_2}]$ contains $\{w_1,w_2,v_1,\ldots,v_m\}$.
                \manolis{Instead of that, would it not be simpler to say that one vertex of $\{w_1, w_2\}$ belongs to $B^\downarrow_{t_1} \setminus B_t$ and the other to $B^\downarrow_{t_2} \setminus B_t$?}
            \end{itemize}
        \end{definition}


        On a high level, given a cycle in $G[B_t^{\downarrow} \setminus \bar{S}]$,
        a swap is happening between two of its vertices when (i) said vertices belong to bla,
        and (ii) any vertex appearing in-between them in the cycle belongs to $B_t$.


        Let $w_1-v_1-\ldots-v_m - w_2$ as in \cref{definition:swap}, such that a swap happens between $w_1$ and $w_2$.
        In the following we argue that one vertex of $\{w_1, w_2\}$ belongs to $B^\downarrow_{t_1} \setminus B_t$ and
        the other to $B^\downarrow_{t_2} \setminus B_t$.
        We first show that $\{w_1,w_2\} \cap B_t = \varnothing$.
        Assume without loss of generality that $w_1 \in B_t$
        and let $w_2 \in B_{t_i}^{\downarrow}$ for some $i \in \{1,2\}$,
        with $B_t \subseteq B_{t_i}^{\downarrow}$.
        Then, it follows that there exists a connected component of $G[B_{t_i}^{\downarrow} \setminus \bar{S_i}]$
        that contains $\{w_1,w_2,v_1,\ldots,v_m\}$, which contradicts the assumption that a swap happens between $w_1$ and $w_2$.
        Furthermore, if $w_1, w_2 \in B^\downarrow_{t_i}$ for some $i \in \{1,2\}$,
        it holds that there exists a component of $G[B^\downarrow_{t_i}\setminus \bar{S_i}]$
        containing $\{w_1,w_2,v_1,\ldots,v_m\}$, a contradiction.


        We are now ready to move on to our proof.
        For the sake of contradiction, assume that $G[B_t^{\downarrow} \setminus \bar{S}]$ contains a cycle,
        and let $\mathcal{C}$ denote one such cycle with a minimum number of swaps,
        where $V(\mathcal{C})$ denotes its vertex set.
        Notice that $\mathcal{C}$ contains vertices from both $B_{t_1}^{\downarrow} \setminus B_t$ and
        $B_{t_2}^{\downarrow} \setminus B_t$,
        as otherwise it exists in either $G[B^\downarrow_{t_1} \setminus \bar{S}]$ or $G[B^\downarrow_{t_2} \setminus \bar{S}]$,
        contradicting the assumption that $(t_1,\bar{S_1},\bar{C_1})$ and $(t_2,\bar{S_2},\bar{C_2})$ are valid partial solutions.

    
        Let $\tau$ denote the number of swaps happening between vertices of $\mathcal{C}$;
        since $\mathcal{C}$ contains vertices from both $B^\downarrow_{t_i} \setminus B_{t_i}$ where $i \in \{1,2\}$,
        it follows that $\tau \ge 2$.
        For $i \in [\tau]$,
        let $(w_{i,1}, w_{i,2})$ denote the pairs of vertices in $\mathcal{C}$ between of which the swaps are happening,
        indexed by their order of appearance;
        \manolis{notice that for all $i \in [\tau]$, there exists a $j \in \{1,2\}$ such that $w_{i,2}, w_{(i \bmod \tau)+1,1} \in B^\downarrow_{t_j} \setminus B_{t_j}$,
        that is, both vertices belong to the same subtree defined by the node $t_j$.}
        Also, let for $i \in [\tau]$, $x_i \in B_t$ denote the first vertex in the path between $w_{i,1}$ and $w_{i,2}$,
        and $P_i$ be the path between $x_i$ and $x_{(i \bmod \tau)+1}$.
        In that case, $\mathcal{C}$ can be obtained from $x_1-P_1-\ldots -x_\tau - P_\tau$.
        Below, we will use $V(P_i)$ to denote the vertex set of the path $P_i$, for every $i \in [\tau]$. 
        

        \begin{observation}
            Every path $P_i$, for $i \in [\tau]$,
            includes a vertex from $B^\downarrow_t \setminus B_t$.
            Also, for every $i \in [\tau]$ and $j \in [2]$,
            $V(P_i) \cap (B^\downarrow_{t_j} \setminus B_{t_j}) \neq \varnothing$
            if and only if $V(P_i) \subseteq B^\downarrow_{t_j} \setminus (B_{t_j} \bar{S_j})$ \manolis{???}.
            \manolis{I think it holds that $V(P_i) \subseteq B^\downarrow_{t_j} \setminus \bar{S_j}$ iff $w_{i,2} \in B^\downarrow_{t_j} \setminus (B_{t_j} \cup \bar{S_j})$. I suggest we write something like this instead, as it is simpler.}
        \end{observation}
        
        To see why the previous holds someone need to consider the definition of the swaps,
        $x_i$'s and $P_i$'s, and recall that $V (\mathcal{C})\subseteq B_t\setminus \bar{S}$.  
        Because of the previous observation, we can also conclude the following.
        \manolis{To conclude the following, we don't need the previous observation, just the fact that the number of swaps is reduced.}
    
        \begin{observation}
            For every pair $x_i, x_{(i \bmod \tau)+1}$, there is no path $q_i$ that connects $x_i$ and $x_{(i \bmod \tau)+1}$ and uses only vertices from $B_{t}\setminus \bar{S}$.
            \manolis{I think that we can say something even stronger: if $w_{i,2} \in B^\downarrow_{t_j} \setminus \bar{S_j}$,
            then there is no path connecting $x_i, x_{(i \bmod \tau)+1}$ using only vertices of $B^\downarrow_{t_{j'}} \setminus \bar{S_{j'}}$,
            where $j' \in \{1,2\} \setminus \{j\}$;
            if that were the case, we could decrease the number of swaps, a contradiction.}
        \end{observation}
    
        Indeed, since the paths $p_i$ and $q_i$ are not identical ($V(q_i)\subseteq B_t$ and $V(p_i)\not\subseteq B_t$) and $V(q_i)\cup V(p_i) \cup \{x_i, x_{(i \bmod \tau)+1}\} \subseteq B^\downarrow_{t_j}\setminus \bar{S_j}$, for some $j \in [2]$ we can conclude that there exists a cycle in $G[B^\downarrow_{t_j}\setminus \bar{S_j}]$. This contradicts to the assumption that $\bar{S_1}$ and $\bar{S_2}$ are feedback vertex sets of $G[B^\downarrow_{t_1}]$ and $G[B^\downarrow_{t_2}]$ respectively.
        \manolis{I don't think we need this proof; it suffices to say that if that were the case, then we could obtain a cycle with a
        smaller number of swaps, a contradiction. }
    

        We now show that there exists a cycle in $G[B^\downarrow_t \setminus S]$, leading to a contradiction.
        Consider the paths $\bar{P_1} = x_1-P_1-x_2$ and $\bar{P_2} =x_2-P_2-\ldots - x_\tau -P_\tau-x_1$. 
        We will show that we can use $\bar{P_1}$ and $\bar{P_2}$ to construct two distinct paths $P'_1$ and $P'_2$ between
        $x_1$ and $x_2$ in $G[B^\downarrow_t \setminus S]$.
        Without loss of generality let $P_1 \subseteq B^\downarrow_{t_1} \setminus \bar{S_1}$. 
        Then, $P_{i} \subseteq B^\downarrow_{t_j} \setminus \bar{S_j}$ if and only if $2 - (i \bmod 2) = j$.
        \manolis{I have no idea what is going on in the previous sentence. From my understanding,
        it holds that $V(P_i) \subseteq B^\downarrow_{t_j} \setminus \bar{S_j}$ iff $w_{i,2} \in B^\downarrow_{t_j} \setminus \bar{S_j}$ though.
        I think you mean to say that in that case for odd indices the paths $P_i$ use vertices of $B^\downarrow_{t_1} \setminus \bar{S_1}$,
        and for even of $B^\downarrow_{t_2} \setminus \bar{S_2}$, but I am not sure and it is written in a confusing way.}
        Indeed, if for some $i \in [\tau]$ and $j \in [2]$, $V(P_i) \subseteq B^\downarrow_{t_j}\setminus \bar{S_j}$ and $V(P_{(i \bmod \tau)+1}) \subseteq B^\downarrow_{t_j}\setminus \bar{S_j}$ then the path $x_1 - P_i - x_{(i \bmod \tau)+1} - P_{(i \bmod \tau)+1}$ uses only vertices of $B^\downarrow_{t_j}$, which contradicts to the definition of $x_{(i \bmod \tau)+1}$.
        \manolis{This contradicts to the fact that a swap $(w_{(i \bmod \tau)+1,1}, w_{(i \bmod \tau)+1,2})$ happens, no?
        Also, $x_1 - P_i - x_{(i \bmod \tau)+1} - P_{(i \bmod \tau)+1}$ is not a path, as $x_1$ does not have an edge with the endpoint of $P_i$.}

        \todo[inline]{\manolis{Up to here.}
        \manolis{Changes: $k \to \tau$; $k$ is used in the definition of the problem.
        $p_i \to P_i$; unusual not to refer to a vertex when using non capitals,
        $P_i \to P'_i$}}

        For each $i \in [k]$ let $\bar{U_i}$ be the connected component of $G[B^\downarrow_{t_{2-(i \bmod 2)}}\setminus \bar{S_{2-(i \bmod 2)}}]$ such that $p_i \subseteq \bar{U_i}$. Because $(t_1,\bar{S_1},\bar{C_1})$ has the same type as $(t_1,S_1,C_1)$, for each $i \in [k]$ such that $i \bmod \tau = 1$, there exists a connected component $U_i$ of $G[B^\downarrow_{t_1}\setminus S_{1}]$ such that $U_i \cap B_{t_1} = U_i \cap B_{t}= \bar{U_i} \cap B_{t} = \bar{U_i} \cap B_{t_1}$. Similarly, since $(t_2,\bar{S_2},\bar{C_2})$ has the same type as $(t_2,S_2,C_2)$, for each $i \in [k]$ such that $i \bmod \tau = 0$, there exists a connected component $U_i$ of $G[B^\downarrow_{t_2}\setminus S_{2}]$ such that $U_i \cap B_{t_2} =  U_i \cap B_{t}= \bar{U_i} \cap B_{t} =\bar{U_i} \cap B_{t_2}$. 
        Notice that we can also conclude that $k$ is even. Indeed, otherwise $p_k - x_1 - p_1$ is a path in $G[B^\downarrow_{t_1}\setminus \bar{S_1}]$ which contradicts to the definition of $x_1$.
    
        Since $x_i-p_i-x_{(i \bmod \tau)+1}$ is a path in $G[B^\downarrow_{t_{2-(i \bmod \tau)}}\setminus S_{2-(i \bmod \tau)}]$ and $V(p_i) \subseteq \bar{U_i}$ we have that $\{x_i,x_{(i \bmod \tau)+1}\}\subseteq \bar{U_i}$. 
        Furthermore, since $\{x_i,x_{(i \bmod \tau)+1}\}\subseteq B_{t}$ we have that $\{x_i,x_{(i \bmod \tau)+1}\}\subseteq U_i$.
        Therefore, for any $i \in [k]$, there exists a path $q_i$ that connects $x_i$ and $x_{(i \bmod \tau)+1}$ in the graph $G[U_i]$. 
        Using the paths $q_i$ instead of $p_i$, for each $i \in [k]$, we are creating two walks $x_1-q_1-x_2$ and $x_2-q_2-\ldots-x_k-q_k-x_1$ in $G[B^\downarrow_t\setminus S]$. Notice that, by construction, $x_1-q_1-x_2$ is a path. Also, the existence of the walk $x_2-q_2-\ldots-x_k-q_k-x_1$ give us a path $x_2-q-x_1$ that uses vertices only from the vertex set $\{x_1\} \cup \bigcup_{i =2}^k (V(p_i)\cup \{x_i\})$. It remains to show that the two paths are not identical. 
    
    
        Notice that, $x_1-q_1-x_2$ uses vertices from $U_1$. Furthermore, by observation \textcolor{red}{blabla} we know that $V(q_1) \setminus B_t \neq \varnothing$. 
        Consider a vertex $x \in V(q_1) \setminus B_t$; we will prove that $x \notin V(q)$. 
        Assume that $x \in V(q)$. 
        Since $x \notin B_t$ and $V(q) \subseteq \{x_1\} \cup \bigcup_{i =2}^k (V(p_i)\cup \{x_i\})$ we have that there exists $i \in [k]\setminus \{1\}$ such that $x \in U_i$. Notice that, since $x \in U_1\setminus B_t$, we have that $U_i = U_1$. Furthermore, since $U_1= U_i \subseteq B^\downarrow_{t_{1}}$. therefore, $i \notin \{2,k\}$ and $k\ge 4$. 
        
        We will use the assumption that $\mathcal{C}$ has minimum number of swaps to show that this can not happen.
        Consider the path $x_2-p_2-\ldots-x_{i-1}p_{i-1}-x_i$. Notice that, since $i\neq 2$, the path  $x_1-p_1-\ldots-x_{i-1}p_{i-1}-x_i$ includes vertices from $B\downarrow_{t_2}\setminus B_{t_2}$ as we have $V(p_2) \subseteq B\downarrow_{t_2}$ and $V(p_2)\not\subseteq B_t$.
        We claim that there exists a path $p$ between $x_1$ and $x_i$ that uses only vertices of $\bar{U_1}$.
        Recall that $U_1\cap B_t = \bar{U_1}\cap B_t$. Also, since $\{x_2,x_i\}\subseteq U_1$ and $\{x_2,x_i\}\subseteq B_t$ we have that $\{x_2,x_i\}\subseteq \bar{U_1}$. Since $\bar{U_1}$ is a connected component of $G[B^\downarrow_{t_1}\setminus \bar{S_1}]$ we have that there exists a path $p$ that connects $x_2$ with $x_i$ and $V(p)\subseteq \bar{U_1}$.
        Therefore, we have two (non identical) paths $x_2-p-x_i$ and $x_2-p_2-\ldots-x_{i-1}-p_{i-1}-x_i$ in $G[B^\downarrow_t\setminus \bar{S}]$ which results to a cycle. Now, notice that the new cycle has less swaps. Indeed, since we have remove all paths $p_j$, $j \in [k]\setminus[i]$ and $i<k$,  we have reduce the swaps by at least $2$. Indeed the cycle we created has at most as many swaps are happening in $x_2-p_2-\ldots p_{i-1}-x_i$ plus two more. This give us at most 
        swaps $i-1$ swaps. However, in $x_1-p_1-\ldots- x_k - p_k$, we have $k>i-1$ swaps; this contradicts to the assumption that $\mathcal{C}$ has a minimum number of swaps. \nikos{I hope that now it is clear... I am not sure who much should I explain the "less swaps" part as for me it is obviously correct but probably extremely technical if we want to define the "new cycle"}
        
        
        
        
    
    \todo[inline]{Nikos: old text in comment}
        \begin{comment}
        Consider a path $v_1 - \ldots - v_{k}$ where $k \ge 3$, $ \{v_1,\ldots,v_{k} \} \cap B_t \setminus \bar{S} =
        \{v_1,v_{k} \}$ and it is part of the cycle $u_1 - \ldots - u_\ell$. 
        Notice that such a path must exist;
        if not, $\{u_1, \ldots, u_\ell\} \in B_t$ and this give a cycle in $G[B_t\setminus S]$.
        \manolis{I do not see why such a path must exist.}
        Fix one such path $v_1 - \ldots - v_{k}$,
        where $\{ v_1,\ldots,v_{k} \} \not\subseteq B_t \setminus S$. 
        It holds that either $\{v_1,\ldots,v_k\} \setminus \{v_1,v_k\} \subseteq B_{t_1}^\downarrow \setminus B_{t_1}$
        or $\{v_1,\ldots,v_k\} \setminus \{v_1,v_k\} \subseteq B_{t_2}^\downarrow \setminus B_{t_2}$,
        as no edges between vertices of $B_{t_1}^\downarrow \setminus B_{t_1}$
        and $B_{t_2}^\downarrow \setminus B_{t_2}$ exist. 
        We will replace $v_1 - \ldots - v_{k}$ with a new path, $p$, between $v_1$ and $v_k$ where all vertices of $p$ are included in $ \{v_1,\ldots,v_{k} \} \not\subseteq B_t\setminus S$.
        \manolis{But the path considered already has this property, no?}
        W.l.o.g. let $\{v_1,\ldots,v_k\} \setminus \{v_1,v_k\} \subseteq B_{t_1}^\downarrow \setminus B_{t_1}$.
        Since $(S_1,C_1)$ and $(\bar{S_1},\bar{C_1})$ have the same type in $t_1$ and
        $\{v_1,v_k\} \subseteq B_{t_1}$,
        the existence of the path $v_1 - \ldots - v_{k}$ in $G[B_{t_1}^\downarrow \setminus \bar{S_1}]$
        means that there exists a path $p$ that connects $v_1$ and $v_k$ in $G[B_{t_1}^\downarrow \setminus S_1]$. 
        By replacing all such paths with the ones which use vertices in $B_{t_1}^\downarrow \setminus S_1$
        or $B_{t_2}^\downarrow \setminus S_2$,
        we create a closed walk in $G[B_t^\downarrow \setminus S]$.
        This contradicts the assumption that $(S,C)$ is a valid partial solution of $t$.
        \manolis{I do not see the contradiction or how we create a closed walk. Have we assumed that $u_1, u_k$ belong to distinct connected components? This proof needs some high level sketch.}
        \end{comment}
    
    \end{claimproof}
